Rust for Embedded Systems: Current State, Challenges and Open Problems (Extended Report)

Embedded software is used in safety-critical systems such as medical devices and autonomous vehicles, where software defects, including security vulnerabilities, have severe consequences. Most embedded codebases are developed in unsafe languages, specifically C/C++, and are riddled with memory safety vulnerabilities. To prevent such vulnerabilities, RUST, a performant memory-safe systems language, provides an optimal choice for developing embedded software. RUST interoperability enables developing RUST applications on top of existing C codebases. Despite this, even the most resourceful organizations continue to develop embedded software in C/C++. This paper performs the first systematic study to holistically understand the current state and challenges of using RUST for embedded systems. Our study is organized across three research questions. We collected a dataset of 2,836 RUST embedded software spanning various categories and 5 Static Application Security Testing ( SAST) tools. We performed a systematic analysis of our dataset and surveys with 225 developers to investigate our research questions. We found that existing RUST software support is inadequate, SAST tools cannot handle certain features of RUST embedded software, resulting in failures, and the prevalence of advanced types in existing RUST software makes it challenging to engineer interoperable code. In addition, we found various challenges faced by developers in using RUST for embedded systems development.

==> code/lockbuddeadlocks.tex <==
\begin{listing}[tb]
    \begin{minted}[escapeinside=||, fontsize=\footnotesize{}]{rust}
Rust code with 
deadlock bug detectable by lockbud tool.
    \end{minted}
    
    \caption{Example demonstrating deadlock bug detectable by~\lockbud{} tool.\aravind{Shashank, add a deadlock example detectable by lockbud}}
    \label{lst:lockbuddeadlocks}
\end{listing}

==> code/lockbuduseaftefree.tex <==
\begin{listing}[tb]
    \begin{minted}[escapeinside=||, fontsize=\footnotesize{}]{rust}
Rust code with 
use-after-free bug detectable by lockbud tool.
    \end{minted}
    
    \caption{Example demonstrating use-after-free bug detectable by~\lockbud{} tool.\aravind{Shashank, add a use-after-free example detectable by lockbud}}
    \label{lst:lockbuduseafterfree}
\end{listing}

==> code/rudramemorysafetybug.tex <==
\begin{listing}[tb]
    \begin{minted}[escapeinside=||, fontsize=\footnotesize{}]{rust}
Rust code with 
memory safety bug detectable by rudra tool.
    \end{minted}
    
    \caption{Example demonstrating memory safety bug detectable by~\rudra{} tool.\aravind{Shashank, add a memory safety example detectable by rudra}}
    \label{lst:rudramemorysafety}
\end{listing}

==> code/rudrasendsyncbug.tex <==
\begin{listing}[tb]
    \begin{minted}[escapeinside=||, fontsize=\footnotesize{}]{rust}
Rust code with 
incorrect send implementation detectable by rudra tool.
    \end{minted}
    
    \caption{Example demonstrating incorrect send implementation detectable by~\rudra{} tool.\aravind{Shashank, add an incorrect send example detectable by rudra}}
    \label{lst:rudrasendsyncbug}
\end{listing}

==> code/safedropuaf.tex <==
\begin{listing}[tb]
    \begin{minted}[escapeinside=||, fontsize=\footnotesize{}]{rust}
Rust code with 
use-after-free bug detectable by safedrop tool.
    \end{minted}
    
    \caption{Example demonstrating use-after-free bug detectable by~\safedrop{} tool.\aravind{Shashank, add a use-after-free example detectable by safedrop}}
    \label{lst:safedropuaf}
\end{listing}

==> figures/callgraphfigure.tex <==
\begin{figure}
    \centering    
    \includegraphics[width=0.48\textwidth]{images/callgraph.pdf}
    \caption{
        Execution flow (\ie Call graph) of the application in~\lst{lst:src-blinky} demonstrating transition across various layers.
    }
    \Description[ Execution flow (\ie Call graph) of the application in~\lst{lst:src-blinky} demonstrating transition across various layers.]{ Execution flow (\ie Call graph) of the application in~\lst{lst:src-blinky} demonstrating transition across various layers.}
    \label{fig:blinkyCG}
\end{figure}

==> figures/onlineresourcesback.tex <==
\begin{figure*}[ht]
\centering
\scriptsize

% Is Rust Documentation helpful?
\begin{minipage}[b]{0.2\linewidth}
%\centering
%\begin{subfigure}[b][0.32\linewidth]
    
\begin{tikzpicture}
\begin{scope}[scale=0.4]
    \pie[text=inside, font=\tiny]{33.3/daddsddsds,33.3/B,33.3/A}
\end{scope}
\end{tikzpicture}
\caption{Is Documentation Helpful?}
    \label{fig:rustdochelpful}
%\end{subfigure}
\end{minipage}

%\hfill
% How can Rust Documentation be improved?
\begin{minipage}[b]{0.2\linewidth}
%\centering
\begin{tikzpicture}
\begin{scope}[scale=0.4]
    \pie[text=inside]{33.3/daddsdssa,33.3/B,33.3/A}
\end{scope}
\end{tikzpicture}
\caption{Suggestions to Improve Documentation}
    \label{fig:rustdocsuggestions}
\end{minipage}

%\hfill
% Refer external resources?
\begin{minipage}[b]{0.2\linewidth}
%\centering
\begin{tikzpicture}%
\begin{scope}[scale=0.4]
    \pie[text=inside]{33.3/daddsdssa,33.3/B,33.3/A}
\end{scope}
\end{tikzpicture}
\caption{Do you refer to external resources?}
\label{fig:rustexternalresources}
\end{minipage}

%\hfill
% Support for rust in community?
\begin{minipage}[b]{0.2\textwidth}
%\centering
\begin{tikzpicture}%
\begin{scope}[scale=0.4]
    \pie[text=inside]{33.3/daddsdssa,33.3/B,33.3/A}
\end{scope}
\end{tikzpicture}
\caption{Support for~\rust in Embedded Systems Community}
\label{fig:rustembeddeddevsupport}
\end{minipage}

\caption{Developers perspective on~\rust{} documentation and community support. \aravind{Shashank: Can you make these figures horizontally aligned.}}
\label{fig:onlineresourcesandcommunitysupport}
\Description[Developers perspective on~\rust{} documentation and community support.]{Developers perspective on~\rust{} documentation and community support.}
\end{figure*}

==> figures/sizeboxplot.tex <==
\pgfplotsset{
     box plot width/.initial=1em,
     box plot/.style={
        /pgfplots/.cd,
        black,
        only marks,
        mark=-,
        mark size=\pgfkeysvalueof{/pgfplots/box plot width},
        /pgfplots/error bars/.cd,
        y dir=plus,
        y explicit,
     },
     box plot box/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \draw  ##1 -- ++(\pgfkeysvalueof{/pgfplots/box plot width},0pt) |- ##2 -- ++(-\pgfkeysvalueof{/pgfplots/box plot width},0pt) |- ##1 -- cycle;
        },
        /pgfplots/table/.cd,
        y index=2,
        y error expr={\thisrowno{3}-\thisrowno{2}},
        /pgfplots/box plot
     },
     box plot top whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=4,
        y error expr={\thisrowno{2}-\thisrowno{4}},
        /pgfplots/box plot
     },
     box plot bottom whisker/.style={
        /pgfplots/error bars/draw error bar/.code 2 args={%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark}%
            {\pgfplotserrorbarsmark}%
            \pgfkeysgetvalue{/pgfplots/error bars/error mark options}%
            {\pgfplotserrorbarsmarkopts}%
            \path ##1 -- ##2;
        },
        /pgfplots/table/.cd,
        y index=5,
        y error expr={\thisrowno{3}-\thisrowno{5}},
        /pgfplots/box plot
     },
     box plot median/.style={
        /pgfplots/box plot
     }
    }
\begin{figure}[h]
\centering
    \begin{tikzpicture}
    \begin{axis} [symbolic x coords={MCUs,Crn,Cre,RRTnr,RRTr}, 
    xtick=data,     
    ylabel=Size (KB),
    ylabel style={font=\footnotesize},
    ytick={0.250, 16, 256},
    %xlabel=Entities,
    xmajorgrids={true},
    height=5cm,
    width=7cm,
    axis background/.style={fill=gray!5},
    xlabel style={font=\footnotesize},
    box plot width=0.5em]
    \addplot [box plot median] table[col sep=comma] {data/sizeplotdata.txt};
     \addplot [box plot box] table[col sep=comma] {data/sizeplotdata.txt};
     \addplot [box plot top whisker] table[col sep=comma] {data/sizeplotdata.txt};
     \addplot [box plot bottom whisker] table[col sep=comma] {data/sizeplotdata.txt};
     \draw[dashed, red] (axis cs:MCUs, 16.000) -- (axis cs:RRTr, 16.000);
    \end{axis}
    \end{tikzpicture}
    \caption{Statistics of sizes of~\acp{MCU} and various~\rust{} software.}
\label{fig:mcusizeboxplot}
\Description[Statistics of sizes of~\acp{MCU} and various~\rust{} software.]{Statistics of sizes of~\acp{MCU} and various~\rust{} software.}
\end{figure}

==> figures/studydesign.tex <==
% https://drive.google.com/file/d/1SXm4gtWR7y1ixjz732iTGUMSgSMHg8q1/view?usp=sharing
\begin{figure}[tb]
    \Description[Overview of study]{Overview of study}
    \centering
    \includegraphics[width=0.46\textwidth]{images/ruststudy.pdf}
    \caption{Overview of our study.\machiry{Fix the Section numbers, finding numbers, and open problem numbers.}}
    \label{fig:ruststudy}
\end{figure}

==> listings/CoR_rust_function_calling_C.tex <==
\begin{listing}[tb]
    \begin{minted}[fontsize=\scriptsize, breaklines]{rust}
extern "C" {
    fn blinky();
}
...
...
#[interrupt]
fn GPIOTE() {
    let p = hal::pac::Peripherals::take().unwrap();
    let port0 = hal::gpio::p0::Parts::new(p.P0);
    //let button = port0.p0_11.into_pullup_input();
    //let led = port0.p0_13.into_push_pull_output(Level::Low);
    unsafe {
        blinky();
    }
}
    \end{minted}
    \caption{Rust calling a C function blinky()}
    \label{lst:rocruststruct}
\end{listing}

==> listings/FreeRTOS_scheduler.tex <==
\begin{listing}[tb]
    \begin{minted}[fontsize=\scriptsize, breaklines]{rust}

extern "C" {
pub fn xTaskCreate(
    pxTaskCode: TaskFunction_t,
    pcName: *const cty::c_char,
    usStackDepth: u16,
    pvParameters: *mut cty::c_void,
    uxPriority: UBaseType_t,
    pxCreatedTask: *mut TaskHandle_t,
) -> BaseType_t;
}
extern "C" {
pub fn vTaskStartScheduler();
}
#[no_mangle]
pub extern "C" fn entry() {
    let task1: core::option::Option<unsafe extern "C" fn(arg1: *mut core::ffi::c_void)>=   Some(vTask1);
    let tn1 = core::str::from_utf8(b"Task 1\0").unwrap().as_ptr() as u8;
    unsafe {
        xTaskCreate(task1, &tn1, 1000, ::core::ptr::null_mut(), 1,::core::ptr::null_mut());
        vTaskStartScheduler();
    }
}
    \end{minted}
    \caption{Rust code snippet to call FreeRTOS scheduler}
    \label{lst:FreeRTOS_scheduler}
\end{listing}    
    

==> listings/Lilos_scheduler.tex <==
\begin{listing}[tb]
    \begin{minted}[fontsize=\scriptsize, breaklines]{rust}
...
pub fn run_tasks(
    futures: &mut [Pin<&mut dyn Future<Output = Infallible>>],
    initial_mask: usize,
) -> ! {
    ...
}
    \end{minted}
    
    \caption{\ac{FFI} incompatible function in Lilos}
    \label{lst:Lilos_scheduler}
\end{listing}

\iffalse
\begin{listing}[tb]
    \begin{minted}[fontsize=\scriptsize, breaklines]{rust}
use core::convert::Infallible;
use core::future::Future;
use core::pin::Pin;
...
...
pub fn run_tasks(
    futures: &mut [Pin<&mut dyn Future<Output = Infallible>>],
    initial_mask: usize,
) -> ! {
    unsafe {
        run_tasks_with_preemption_and_idle(
            futures,
            initial_mask,
            Interrupts::Masked,
            || {
                cortex_m::asm::wfi();
                cortex_m::asm::isb();
            },
        )
    }
}
    \end{minted}
    
    \caption{Lilos scheduler}
    \label{lst:Lilos_scheduler}
\end{listing}
\fi

==> listings/RoC_C_struct.tex <==
\begin{listing}[tb]
    \begin{minted}[fontsize=\scriptsize, breaklines]{rust}
#[repr(C)]
#[derive(Copy, Clone)]
pub struct NRF_GPIO_Type {
    pub RESERVED: [u32; 321usize],
    pub OUT: u32,
    pub OUTSET: u32,
    pub OUTCLR: u32,
    pub IN: u32,
    pub DIR: u32,
    pub DIRSET: u32,
    pub DIRCLR: u32,
    pub LATCH: u32,
    pub DETECTMODE: u32,
    pub RESERVED1: [u32; 118usize],
    pub PIN_CNF: [u32; 32usize],
}  
    \end{minted}
    
    \caption{NRF\_GPIO\_Type C struct converted to Rust  }
    \label{lst:roccstruct}
\end{listing}

==> listings/RoC_rust_func.tex <==
\begin{listing}[tb]
    \begin{minted}[fontsize=\scriptsize, breaklines]{rust}
#[no_mangle]
pub unsafe extern "C" fn togglePin(pin_num: u32) {
    // Cast the address to a mutable reference of NRF_GPIO_Type
    let gpio: &mut NRF_GPIO_Type = unsafe { &mut *(NRF_P0_BASE as *mut NRF_GPIO_Type) };
    // Toggle the specific pin in the OUT field
    let pins_state = gpio.OUT;
    gpio.OUTSET = !pins_state & (1 << pin_num);
    gpio.OUTCLR = pins_state & (1 << pin_num);
}
    \end{minted}
    
    \caption{Rust Function which interacts with FreeRTOS to toggle led using C APIs}
    \label{lst:rocrustfunc}
\end{listing}

==> listings/lockbugrealbug.tex <==
\begin{listing}[tb]
    \begin{minted}[escapeinside=||, fontsize=\footnotesize{}]{rust}
fn execute_write(&self, ...) -> RspResult<Rsp> {
    ...
    // first lock happens here. |\textcolor{yellow}{\faLock}|
    let mut cc = self.cc.lock();
    ...
    for (hdl, off, val) in cc.write_queue.iter() {
      (w.hdl, w.uuid, w.off, w.val) = (
                        hdl, self.uuid(hdl), off, val);
      // calls do_write()
      self.do_write(&w)?;
         // this will eventually call
         // self.cc.lock();|\textcolor{red}{\faLock}|
    ...
    \end{minted}
    
    \caption{Deadlock (\textcolor{red}{\faLock}) found by~\lockbud{} in~\code{burble} crate.}
    \label{lst:lockbudrealbug}
\end{listing}

==> listings/nostdconversion.tex <==
% \begin{listing*}[t!]
%   \begin{tabular}{c|c|c}
%     \begin{minipage}{.25\textwidth}
% % \inputminted[xleftmargin=20pt,linenos, mathescape, escapeinside=||, fontsize=\scriptsize{}]{rust}{code/ex-orig.rs}
%     \begin{minted}[fontsize=\scriptsize, breaklines]{rust}
% // Existing std compatible code
% use std::fs;
% use std::io;

% struct Foo {
%     map: std::collections::HashMap<i32, Vec<i32>>,
% }

% fn bar() -> Foo {
%     println!("hello world");

%     let _ = log_message("some message");

%     Foo{
%         map: Default::default()
%     }
% }

% fn log_message(msg: &str) -> io::Result<Vec<u8>> {
%     let data = fs::read("somefile.txt")?;
%     Ok(data)
% }

% // ========================================
% // After conversion to be no

% #![cfg_attr(not(feature = "std"), no_std)]

% extern crate alloc;

% #[cfg(feature = "std")]
% use std::fs;
% #[cfg(feature = "std")]
% use std::io;

% struct Foo {
%     #[cfg(feature = "std")]
%     map: std::collections::HashMap<i32, alloc::vec::Vec<i32>>,

%     #[cfg(not(feature = "std"))]
%     map: hashbrown::HashMap<i32, alloc::vec::Vec<i32>>
% }

% fn bar() -> Foo {
%     #[cfg(feature = "std")]
%     println!("hello world");

%     #[cfg(feature = "std")]
%     let _ = log_message("some message");

%     Foo{
%         map: Default::default()
%     }
% }

% #[cfg(feature = "std")]
% fn log_message(msg: &str) -> io::Result<Vec<u8>> {
%     let data = fs::read("somefile.txt")?;
%     Ok(data)
% }
%     \end{minted}
%     \end{minipage}
%   \end{tabular}
% \caption{Example demonstrating some of the changes involved in converting Rust~\rustcode{std} code to~\rustcode{no_std}}
% \label{lst:nostdconversion}
% \end{listing*}

\begin{listing}[tb]
    \begin{minted}[fontsize=\scriptsize, breaklines]{rust}
// Existing std compatible code
use std::fs;
use std::io;

struct Foo {
    map: std::collections::HashMap<i32, Vec<i32>>,
}

fn bar() -> Foo {
    println!("hello world");

    let _ = log_message("some message");

    Foo{
        map: Default::default()
    }
}

fn log_message(msg: &str) -> io::Result<Vec<u8>> {
    let data = fs::read("somefile.txt")?;
    Ok(data)
}

// ========================================
// After conversion to be no

#![cfg_attr(not(feature = "std"), no_std)]

extern crate alloc;

#[cfg(feature = "std")]
use std::fs;
#[cfg(feature = "std")]
use std::io;

struct Foo {
    #[cfg(feature = "std")]
    map: std::collections::HashMap<i32, alloc::vec::Vec<i32>>,

    #[cfg(not(feature = "std"))]
    map: hashbrown::HashMap<i32, alloc::vec::Vec<i32>>
}

fn bar() -> Foo {
    #[cfg(feature = "std")]
    println!("hello world");

    #[cfg(feature = "std")]
    let _ = log_message("some message");

    Foo{
        map: Default::default()
    }
}

#[cfg(feature = "std")]
fn log_message(msg: &str) -> io::Result<Vec<u8>> {
    let data = fs::read("somefile.txt")?;
    Ok(data)
}
    \end{minted}
    \caption{Example demonstrating some of the changes involved in converting Rust~\rustcode{std} code to~\rustcode{no_std}}
    \label{lst:nostdconversion}
\end{listing}

==> listings/rustcbindings.tex <==
extern "C" {
    pub fn add(a: ::std::os::raw::c_int, b: ::std::os::raw::c_int) -> ::std::os::raw::c_int;
}

==> listings/safedroprealbug.tex <==
\begin{listing}[tb]
    \begin{minted}[escapeinside=||, fontsize=\footnotesize{}]{rust}
extern "C" fn sys_ipc_publish(
  ..., msg_ptr: *mut u8, ...) -> usize {
  unsafe {
    // vec created from raw pointer |\textcolor{yellow}{\faWarning}|
    let msg_vec = Vec::from_raw_parts(
      msg_ptr, msg_len, msg_len
    );
    ...
      Err(_) => {
        // another vec created from the 
        // same raw pointer |\textcolor{yellow}{\faWarning}|
        Vec::from_raw_parts(msg_ptr, msg_len, msg_len);
        return 1;
        // both first and second vec will be 
        // dropped, resulting in double-free |\textcolor{red}{\faBug}|
      }
    \end{minted}
    
    \caption{Double-free bug found by~\safedrop{} in~\code{fe_rtos} crate.}
    \label{lst:safedroprealbug}
\end{listing}

==> sections/motivation.tex <==
\section{Motivation}
\label{sec:motivation1}
%\input{tables/bugtable}
Our analysis (details in~\apdx{apdx:rtosbugstudy}) of security vulnerabilities in various~\acp{RTOS} (an important class of embedded software) for the past ten years shows that 59 (54.2\%) of them are memory corruption vulnerabilities,~\ie spatial or temporal memory issues.
%
%As mentioned in~\sect{subsec:embeddedsystems}, in type-2 systems, all tasks (including~\ac{RTOS}) and other layers (\fig{fig:background}) execute in a single address space~\cite{mariusndsspaper}.
%In other words, a task can access entire memory.
%A memory corruption bug in a task can be used to gain complete control of the system,~\eg{} an arbitrary write vulnerability in a task can be exploited to modify the code of other tasks or structures maintained by the underlying~\ac{RTOS}.

%Hardware mechanisms needed for exploit hardening mechanisms (\ie{}~\ac{DEP}~\cite{microsoft2018data} and~\ac{ASLR}~\cite{snow2013just}) such as~\ac{MMU} and~\ac{MPU} are either missing in most~\acp{MCU} or hard to use them in practice~\cite{mpuusagewild, yu2022building}.
%Exploit hardening mechanisms, such as~\ac{DEP}~\cite{microsoft2018data} and~\ac{ASLR}~\cite{snow2013just}, need hardware support (such as~\acp{MMU}) which is missing in most~\acp{MCU}.
%Although recent~\acp{MCU} contain~\acf{MPU} (a less powerful~\ac{MMU}), it is hard to use them on existing~\ac{RTOS} and consequently, developers frequently use them improperly~\cite{mpuusagewild} --- rendering them useless in practice.
%Finally, even if hardware mechanisms exist, other challenges with legacy embedded systems make it hard for developers to use them in their development lifecycle~\cite{yu2022building}.

\iffalse
To understand common security issues in embedded systems, we collected publically reported vulnerabilities from the CVE database~\cite{noauthor_cve_nodate} across various~\acp{RTOS} --- the important component of type-2 systems.\santiago{Can we make any claims as to this sample being representative? can we elaborate on time windows of these vulnerabilities? (e.g., it'd be very bad if all of these CVEs were from 2014 and there is nothing recent)} 

\subsection{Vulnerabilities Study}
We focused on vulnerabilities with the necessary technical details to understand the root cause; this resulted in a total of 109 vulnerabilities.
We manually categorized each of them according to their root cause,~\tbl{tab:bugsinrtos} shows the categorization.
%of these vulnerabilities according to their root causes.
There are 25 (22.9\%) application-specific vulnerabilities that any programming language cannot prevent.
However, there are 59 (54.2\%) memory corruption vulnerabilities,~\ie spatial or temporal memory issues.


\subsection{Lack of Security Mechanisms}
Exploit hardening mechanisms, such as~\ac{DEP}~\cite{microsoft2018data} and~\ac{ASLR}~\cite{snow2013just}, use various tricks to make exploitation of these vulnerabilities hard.
However, most~\acp{MCU} lack~\acf{MMU}~\cite{milenkovic1990microprocessor} and do not have the support for virtual address and other memory protection mechanisms.
This lack of hardware support makes it challenging to have common exploit-hardening mechanisms. 
Although recent~\acp{MCU} contain~\acf{MPU} (a less poweful~\ac{MMU}), it is hard to use them on existing~\ac{RTOS} and consequently, developers frequently use them improperly~\cite{mpuusagewild} --- rendering them useless in practice.
Finally, even if hardware mechanisms exist, other challenges with legacy embedded systems make it hard for developers to use them in their development lifecycle~\cite{yu2022building}.

\subsubsection{No Privilege Separation} 
Unfortunately, in type-2 systems, all tasks (including~\ac{RTOS}) and other layers (\fig{fig:background}) execute in a single address space~\cite{mariusndsspaper}.
In other words, a task can access entire memory.
A memory corruption bug in a task can be used to gain complete control of the system,~\eg, an arbitrary write vulnerability in a task can be exploited to modify the code of other tasks or structures maintained by the underlying~\ac{RTOS}.
\fi

%\myparagraph{Need for Memory Safety and~\rust{}}
%\emph{Since most (54.2\%) vulnerabilities are memory issues, using memory-safe languages is another way to prevent them.}
It is important to use memory-safe languages to prevent such vulnerabilities.
%is another way to prevent them
%These vulnerabilities can be prevented by using memory-safe programming languages.
%\emph{This shows that the most commonly occurring vulnerabilities in embedded systems can be prevented by using memory-safe programming languages}.
%
%Although many memory-safe languages exist, such as Java, Python, Go, etc,
\rust{}, a memory-safe language with its superior performance, has been considered best suited for C system codebases.
Also,~\rust{} has been increasingly adopted by large organizations such as Google~\cite{noauthor_google_nodate} and Microsoft~\cite{claburn_microsoft_nodate} and is used in non-embedded environments.% operating systems.
The lack of~\ac{OS} abstractions, the prevalence of asynchronous execution semantics, and the need for low-level accesses pose unique challenges to readily adopt~\rust{} for embedded systems.
\emph{It is important to holistically understand the state of~\rust{} ecosystem for embedded system development and what aspects hinder the adoption of~\rust{} to embedded systems and its challenges.}
%Starting 6.1, Linux Kernel added support for~\rust{}~\cite{noauthor_rust_nodate-2}.
%Similarly, many projects~\cite{noauthor_android_nodate} in Android use~\rust{}.
%
%\rust{} also has a specific embedded system focus~\cite{noauthor_rust_nodate-1}, and many resources exist that encourage the adoption of~\rust{} to embedded systems.
%A few works~\cite{10.1145/3124680.3124717, Levy2017MultiprogrammingA6} also demonstrated the feasibility of implementing an entire embedded system stack in~\rust{}.
%Despite this, many embedded systems are still developed in C.
%For instance, Microsoft recently released Azure RTOS~\cite{noauthor_azure_nodate}, an~\ac{RTOS} for embedded systems, which is completely developed in C.
%\emph{It is important to holistically understand what aspects hinder the adoption of~\rust{} to embedded systems and its challenges.}
Unfortunately, no systematic studies exist.
%No systematic study exists that analyzes the use of~\rust{} in embedded systems to understand its challenges and shed light on open problems.
%This work fills this gap by performing an organized analysis to answer various research questions related to the use of~\rust{} in embedded systems.

==> sections/rq1applicability.tex <==
\section{RQ1: Applicability of Rust}
\label{subsec:applicabilityofrust}
We want to assess whether~\rust{} is a practical memory-safe language for embedded systems.
As mentioned in~\sect{subsec:embeddedsystems}, these systems have a lot of diversity in hardware (\ie~\acp{MCU}), execute in low-memory environments, and have strict timing requirements (\ie{} real-time constraints).
To assess~\rust{}'s suitability, we need to investigate: (i)~\rust{}'s existing hardware support and ease of adding new targets; (ii) Whether~\rust{} binaries are small enough to fit in a typical~\ac{MCU}, and finally, (ii) Whether the performance of~\rust{} is similar to that of native (\ie C/C++) programs.
\iffalse
Here, we want to assess whether~\rust{} is a practical memory-safe language for embedded systems.
As mentioned in~\sect{subsec:embeddedsystems}, from a software engineering perspective, these systems have the following characteristics: a lot of diversity in hardware (\ie~\acp{MCU}), execute in low-memory environments, and have strict timing requirements (\ie{} real-time constraints).
To be applicable,~\rust{} should satisfy the above requirements.
\fi
\subsection{\texorpdfstring{\rust{}'s Embedded Hardware Support}{Rust's Embedded Hardware Support}}
\label{subsec:rusthardwaresupport}

Hardware support of a compilable programming language (like~\rust{}) comprises two aspects: (i)~\ac{ISA} or Architecture support: Can the compiler generate machine instructions corresponding to the target? (ii) Target or toolchain support: Can the compiler produce a binary executable with valid instructions and data format compatible with a target processor environment?

\noindent\textbf{\ac{ISA} Support:}~\acp{MCU} use~\ac{RISC}~\acp{ISA}, such as ARM.
The~\rust{} compiler~\rustc{}~\cite{rustccompiler} uses~\llvm{} as the backend for machine code generation and consequently,~\rustc{} also supports~\cite{rustccompilersupport} all~\acp{ISA} supported by~\llvm{}.
The recent and stable version of~\llvm,~\ie version 13, supports 38 different~\ac{RISC} architectures, including ARM, MIPS, and RISC-V.
Unfortunately,~\rustc does not have built-in support~\cite{avrrust} for AVR -- one of the common architectures in embedded systems development. However, there are active efforts~\cite{avrrust} to include this.

\noindent\textbf{Target Support:}~\ac{ISA} support does not indicate that the compiler can generate a valid binary for an~\ac{MCU} with the~\ac{ISA}.
A compiler requires various other information (\eg~\ac{ABI} or calling convention) to generate an executable binary from the source code,~\lst{lst:rusttarget} shows an example of the details required to generate ARM v7 firmware. For instance, the key ``data-layout'' represents the layout of various data entities, such as stack alignment (\code{S64})).
\emph{The recent version of~\rustc{} (version: 1.70) supports 29 embedded system targets~\footnote{Computed using \shell{rustc --print target-list}}~\cite{rustcplatformsupport}, including ARM-Cortex-M, Aarch64, ARM, MSP430 --- which are the most popular and commonly used architectures in type-2 embedded systems~\cite{Scharnowski2022FuzzwareUP, 10.5555/3277203.3277227, 8835392, p2im,patterson1980case}}.

%\input{listings/newtargetjson}

\noindent\textbf{Adding New Targets:}
Developers can add support for new targets through an architecture specification~\ie{} a JSON file with all the required information.
The~\lst{lst:rusttarget} from the Appendix shows an example of this.
%An example is shown in~\lst{lst:rusttarget} in Appendix.
Developers can use existing target specifications (using~\shell{--print target-spec-json} command) and tweak them to create new target specifications.
\iffalse
Developers can create a new target using a JSON file with all the required information, as shown in~\lst{lst:rusttarget}.
If the new target is similar to an existing target, the recommended way~\cite{creatingsustomtarget} to create the JSON is to print the existing target spec using~\shell{--print target-spec-json} command.
Second, tweaking the JSON to match the properties of the new target.
\fi

\noindent\textbf{On-going Improvements:} 
%Unfortunately,~\rustc does not have built-in support~\cite{avrrust} for AVR -- one of the common architectures in embedded systems development. However, there are active efforts~\cite{avrrust} to include this.
\gcc{} has more extensive target support for embedded systems.
There is an active effort~\gccrs{}~\cite{gccrs}, where the goal is to use integrate~\rustc{} into~\gcc{}, which also enables the use of extensive GNU tools.

\input{figures/sizeboxplot}

\subsection{\texorpdfstring{Size of~\rust{} Binaries}{Size of Rust Binaries}}
\label{subsec:rustbinarysize}
Embedded systems run on~\acp{MCU} with a small amount of on-device main memory (or RAM).
We analyzed popular~\ac{MCU} boards (\apdx{apdx:macuanalysis}) and found the available memory on these devices ranges from~\minmcumemory{} bytes -~\maxmcumemory{} KB.
The first bar in~\fig{fig:mcusizeboxplot} shows the box plot of memory sizes in~\ac{MCU} boards.
The red-dotted lines across show the median memory size~\ie 16KB.

One of the well-known drawbacks of~\rust is the size of the generated binary. For instance, a simple hello world program in~\rust is 4.1 MB (without debug symbols).
This large size is mainly because the standard library is automatically included in the generated binary.
We can disable this by using~\rust{}'s~\code{no_std} mode, which does not include standard libraries and other startup code.
All embedded software in~\rust{} use~\code{no_std} mode and are considerably small.
The~\rustnonembcrates{}  and~\rustembcrates{} bars in~\fig{fig:mcusizeboxplot} show the box plot of code-section sizes of non-embedded and embedded crates, respectively.
As we can see, embedded crates (\rustembcrates{}) are considerably smaller, with a median size of 10K ($<$ 16K (median MCU memory)).
Similarly, as indicated by~\nonnativerustrots{} and~\nativerustrots{} bars,~\rust{}~\acp{RTOS} are also considerably smaller with a median size of 9K and 8K, respectively.
This shows binaries produced by~\rust{} for embedded software can fit on~\ac{MCU} boards.
Furthermore, there are ongoing works~\cite{ayers2022tighten} that try to further reduce the size of~\rust{} binaries. 

\iffalse
\aravind{Need to clean this up after numbers are filled.}
What is the typical size of available storage (flash) in MCU?

As mentioned before (in background), embedded systems run on microcontroller boards designed to have a low power consumption and usually have limited amount of on-device main memory (or RAM).
We analyzed popular MCU boards (details in appendix) and found the available memory on these devices ranges from: 256 bytes - 512 KB. The first bar in figure shows the box plot of the memory sizes.

What is the average size of rust binary? Regular application and embedded crates?
Size of Rust-based Embedded OSes?

One of the drawbacks of~\rust is the size of the generated binary. For instance, a simple hello world program in C and~\rust is 16 KB and 4.1 MB (without debug symbols), respectively.
To get an better understand of this, we computed the size of regular rust applications, the third bar in fig shows the size ranges.
---talk about the size and compare it with the board sizes---

This large size is mainly because of standard library  (stdlib).
There is embedded rust which avoid this by not including stdlid (nostdlib), enabling development of rust application whose size is comparable to that of regular C/C++ applications.
To evaluate this, we computed the size of~\rustembcrates, the second bar in fig show the box plot.
This shows that it is possible to have a embedded software in rust that can fit on microcontroller boards.
Furthermore, the existence of rust based embedded RTOSes further demonstrates this. \ayushi{We can cite 'Tighten Rust’s Belt: Shrinking Embedded Rust Binaries'\cite{10.1145/3519941.3535075} here?}
\fi
\subsection{\texorpdfstring{Performance of~\rust{}}{Performance of Rust}}
\label{subsec:rustperf}
Several works compare the performance of~\rust{} programs with those written in C/C++.
The results are contradictory.
Few works~\cite{rustvsc,spedofrust} show that~\rust{} programs are as fast or even faster than C/C++ counterparts.
However, recently Zhang~\etal{}~\cite{junperformance} argue that~\rust{} programs are consistently slower.
Furthermore, the conclusions of these studies change as~\rustc evolves with more optimizations.

The main reasons for performance overhead (if any) in~\rust{} is because of using~\texttt{std} library and additional runtime checks.
However, embedded software in~\rust{} is compiled with~\code{no_std} mode, which does not include ~\texttt{std} library and has all many checks disabled~\cite{rustonmicro}.
Several~\rust{} based~\acp{RTOS} are developed (\sect{subsec:rustbinarysize}) based on this and have performance comparable to traditional~\acp{RTOS}.
However,~\emph{no existing study systematically tries to evaluate~\rust{}'s performance on embedded systems}.


\begin{tcolorbox} [width=\linewidth, colback=yellow!30!white, top=1pt, bottom=1pt, left=2pt, right=2pt]
\textbf{Finding RQ1.1 (\sect{subsec:rusthardwaresupport}):} 
The architecture support by~\rust{} is adequate for embedded systems (\sect{subsec:rusthardwaresupport}).
Although AVR is not readily supported, there are promising ongoing efforts to improve this.

\textbf{Finding RQ1.2 (\sect{subsec:rustbinarysize}):}
\rust{}'s~\code{no_std} mode enables generation of smaller binaries which can fit into most~\acp{MCU} memory.
 
\textbf{Finding RQ1.3 (\sect{subsec:rustperf}):}
There are high-performant configurations (\code{no_std}) of~\rust{}, which results in performance similar to that of native programs. However, no work exists that tries to do a systematic performance evaluation of~\rust{} embedded systems.

\end{tcolorbox}

==> tables/c2rustblinky.tex <==
\begin{table}[]
\caption{Results of converting sample C RTOS applications to Rust using c2rust.\santiago{I wonder how difficult it is to do this with TI-RTOS}}
\label{tab:c2rustblinky}
\scriptsize
\centering
{\color{blue} % begin color
\begin{tabular}{llccl}
\toprule
\textbf{S.No.} & \textbf{RTOS Name}             & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}l@{}}c2rust \\ transpilation\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}l@{}}Transpiled \\ project \\ builds?\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}Overall \\ Result\end{tabular}} \\ \midrule
1 & RT-Thread/rt-thread             & Success$^*$   & Failed    & Failed  \\ \midrule
2 & zephyrproject-rtos/zephyr       & Failed        & NA        & Failed  \\ \midrule
3 & RIOT-OS/RIOT                    & Failed        & NA        & Failed  \\ \midrule
4 & seL4/seL4                       & Failed        & NA        & Failed  \\ \midrule
5 & FreeRTOS/FreeRTOS               & Success$^*$   & Failed    & Failed  \\ \midrule
6 & azure-rtos/threadx              & Success$^*$   & Failed    & Failed  \\ \midrule
7 & apache/nuttx                    & Success$^*$   & Failed    & Failed  \\ \midrule
8 & contiki-ng/contiki-ng           & Success$^*$   & Failed    & Failed  \\ \midrule
9 & embox/embox                     & Failed        & NA        & Failed  \\ \midrule
10 & TrampolineRTOS/trampoline      & Success$^*$   & Failed    & Failed  \\ \midrule
11 & kelvinlawson/atomthreads       & Success       & Failed    & Failed  \\ \midrule
12 & insane-adding-machines/frosted & Success$^*$   & Failed    & Failed  \\ \midrule
13 & echronos/echronos              & Success       & Failed    & Failed  \\ \midrule
14 & jameswalmsley/bitthunder       & Failed        & NA        & Failed  \\ \midrule
15 & stateos/StateOS                & Failed        & NA        & Failed  \\ \midrule
16 & kmilo17pet/QuarkTS             & Success$^*$   & Success   & Success \\ 
\bottomrule
\end{tabular}
}  % end color
\end{table}


==> tables/clibwrappers.tex <==
\begin{table}[]
\caption{Percent of Embedded Crates that are wrappers around C libraries. \shank{merge tabl 7 with tab 3. additional seaparator lines to separate wrapper crates}}
\label{tab:clibwrappers}
\footnotesize
\centering
{\color{blue} % color begin
\begin{tabular}{|l|r|r|r|}
\hline
\multicolumn{1}{|c|}{\textbf{Category}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Total \\ Number \\ of Crates\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Numer of \\ Wrapper \\ Crates\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}\% of \\ wrapper \\ crates\end{tabular}}} \\ \hline
RTOS Crates                             & 21                                                                                                 & 10                                                                                                  & 50\%                                                                                             \\ \hline
Driver Crates                           & 444                                                                                                & 100                                                                                                 & 11.11\%                                                                                          \\ \hline
HAL Crates                              & 243                                                                                                & 111                                                                                                 & 11.11\%                                                                                          \\ \hline
Board Support Package                   & 146                                                                                                & 22                                                                                                  & 22.22\%                                                                                          \\ \hline
Peripheral Access Crates                & 641                                                                                                & 33                                                                                                  & 33.33\%                                                                                          \\ \hline
Architecture Support Crates             & 48                                                                                                 & 55                                                                                                  & 55.55\%                                                                                          \\ \hline
Utility Crates                          & 1308                                                                                               & 33                                                                                                  & 33\%                                                                                             \\ \hline
\textbf{Total}                          & \textbf{2851}                                                                                      & \textbf{1000}                                                                                       & \textbf{60.44\%}                                                                                 \\ \hline
\end{tabular}
} % color end

\end{table}

==> tables/qrates.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table*}[]
\caption{Qrates results.}
\label{tab:qrates}
\centering
{\color{blue}   % color start
\begin{tabular}{crrrrrrr}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Category}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Num. Crates\\ compiled\end{tabular}}}} & \multicolumn{5}{c}{\textbf{Number of Crates having:}}                                                                                                                                                                                                                                                                                                                              & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}\% of Crates having \\ atleast one of these \\ Unsafe Constructs\end{tabular}}}} \\ \cmidrule(lr){3-7}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{}                                  & \textbf{\begin{tabular}[c]{@{}l@{}}Unsafe \\ Blocks\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Unsafe \\ Functions\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Unsafe Trait \\ Impls\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Unsafe \\ Traits\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Atleast one of \\ these Unsafe Cosntructs\end{tabular}} & \multicolumn{1}{c}{}                                                                                                                                   \\ \midrule
\abbrrtoscr     & \perrtoscompiled    & \numrtosub    & \numrtosuf    & \numrtosuti   & \numrtosut    & \numrtosuatone    & \perrtosuatone    \\ \midrule
\abbrdrivercr   & \perdrivercompiled    & \numdriverub    & \numdriveruf    & \numdriveruti   & \numdriverut    & \numdriveruatone    & \perdriveruatone    \\ \midrule
\abbrhalcr      & \perhalcompiled    & \numhalub    & \numhaluf    & \numhaluti   & \numhalut    & \numhaluatone    & \perhaluatone    \\ \midrule
\abbrbspcr      & \perbspcompiled    & \numbspub    & \numbspuf    & \numbsputi   & \numbsput    & \numbspuatone    & \perbspuatone    \\ \midrule
\abbrpaccr      & \perpaccompiled    & \numpacub    & \numpacuf    & \numpacuti   & \numpacut    & \numpacuatone    & \perpacuatone    \\ \midrule
\abbrarchcr     & \perarchcompiled    & \numarchub    & \numarchuf    & \numarchuti   & \numarchut    & \numarchuatone    & \perarchuatone    \\ \midrule
\abbrutilcr     & \perutilcompiled    & \numutilub    & \numutiluf    & \numutiluti   & \numutilut    & \numutiluatone    & \perutiluatone    \\
\bottomrule
\end{tabular}
}   % color end
\end{table*}


==> tables/qrates_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\caption{Qrates results. \shank{make this take whole page width. abbr. category breakup. number and percentage having atleast 1 of these issues.}}
\label{tab:qrates}
\small
\centering
{\color{blue} % being color
\begin{tabular}{|l|r|rrllll|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{Category}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Total \\ Number \\ of Crates\end{tabular}}}} & \multicolumn{6}{c|}{\textbf{Number of Crates having:}}                                                                                                                                                                                                                                                                                                                                                                                                                      \\ \cline{3-8} 
\multicolumn{1}{|c|}{}                                   & \multicolumn{1}{c|}{}                                                                                               & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}No\\ Unsafe\end{tabular}}} & \multicolumn{1}{l|}{\textbf{Unsafe}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Unsafe\\ Blocks\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Unsafe\\ Functions\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Unsafe\\ Trait Impls\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}Unsafe\\ Traits\end{tabular}} \\ \hline
RTOS Crates                                              & 21                                                                                                                  & \multicolumn{1}{r|}{10}                                                           & \multicolumn{1}{r|}{11}              & \multicolumn{1}{l|}{}                                                                 & \multicolumn{1}{l|}{}                                                                    & \multicolumn{1}{l|}{}                                                                      &                                                                  \\ \hline
Driver Crates                                            & 444                                                                                                                 & \multicolumn{1}{r|}{100}                                                          & \multicolumn{1}{r|}{333}             & \multicolumn{1}{l|}{}                                                                 & \multicolumn{1}{l|}{}                                                                    & \multicolumn{1}{l|}{}                                                                      &                                                                  \\ \hline
HAL Crates                                               & 243                                                                                                                 & \multicolumn{1}{r|}{111}                                                          & \multicolumn{1}{r|}{222}             & \multicolumn{1}{l|}{}                                                                 & \multicolumn{1}{l|}{}                                                                    & \multicolumn{1}{l|}{}                                                                      &                                                                  \\ \hline
Board Support Package                                    & 146                                                                                                                 & \multicolumn{1}{r|}{22}                                                           & \multicolumn{1}{r|}{66}              & \multicolumn{1}{l|}{}                                                                 & \multicolumn{1}{l|}{}                                                                    & \multicolumn{1}{l|}{}                                                                      &                                                                  \\ \hline
Peripheral Access Crates                                 & 641                                                                                                                 & \multicolumn{1}{r|}{33}                                                           & \multicolumn{1}{r|}{555}             & \multicolumn{1}{l|}{}                                                                 & \multicolumn{1}{l|}{}                                                                    & \multicolumn{1}{l|}{}                                                                      &                                                                  \\ \hline
Architecture Support Crates                              & 48                                                                                                                  & \multicolumn{1}{r|}{55}                                                           & \multicolumn{1}{r|}{5}               & \multicolumn{1}{l|}{}                                                                 & \multicolumn{1}{l|}{}                                                                    & \multicolumn{1}{l|}{}                                                                      &                                                                  \\ \hline
Utility Crates                                           & 1308                                                                                                                & \multicolumn{1}{r|}{33}                                                           & \multicolumn{1}{r|}{77}              & \multicolumn{1}{l|}{}                                                                 & \multicolumn{1}{l|}{}                                                                    & \multicolumn{1}{l|}{}                                                                      &                                                                  \\ \hline
\textbf{Total}                                           & \textbf{2851}                                                                                                       & \multicolumn{1}{r|}{\textbf{1000}}                                                & \multicolumn{1}{r|}{\textbf{800}}    & \multicolumn{1}{l|}{}                                                                 & \multicolumn{1}{l|}{}                                                                    & \multicolumn{1}{l|}{}                                                                      &                                                                  \\ \hline
\end{tabular}
} % end color
\end{table*}

==> toolsummary.tex <==
\section{Tool description}
\begin{itemize}
\item\textbf{\yuga{}~\cite{Nitin2023YugaAD}:}
Life Time annotation bugs
	 - arg-arg  - ex:
	 - arg-return - ex:  RUSTSEC-2021-0130
\textit{Function Signature Lifetime Extraction}
- If value is borrowed with Lifetime - X 
	- All it's fields and values should outlive X
- If value is pointed by raw pointer, raw pointer is in struct
	- Then the value must outlive Lifetime(Struct)
	- If no Lifetime Annotation - then it's considered to be owned by the struct object\\
\textit{Lifetime annotation checking:}
 - check for assignments of
	 - arg to ret: (consider statements dealing with raw pointers). pair arguments and return values.
  \begin{itemize}
      \item - use after free: lifetime arg< lifetime of ret value
       \item - non-exclusive mutability: LA(value) < LA(*mut value/\&mut value )
  \end{itemize}
	
	 - arg to arg
		 - pick two arguments at a time and iterate through all pair of values inside these arguments
			- if the types match then there and either or both of them are mutable, then their could a potential bug if there is lifetime mismatch \\
\textit{Alias checking for Intra procedural stuff:} 
- determine if two pointers point to the same location.
	- three kind of analysis
	- Intra procedural: treat functions as opaque
	- Field sensitive: each field of struct is treated seperately.
	- flow sensitive: this is on intra procedural level.
If we have a = b then we merge b’s points-to set into a’s. flow sensitive because we process each statement just once in order.
ignores analysis of the values whose types are unknown to the pass.
 False Positive Prevention
Reason for false positives: less granularity for intra procedural pointer analysis. fails to differentiate between accesses to elements of same ibject

- use of heuristics to eliminate them

\item\textbf{\rcanary{}~\cite{unknown}:}
detection of leaks that can occur in the semi-automated memory management. lack of manual deallocation while using ManuallyDrop
\_Note:\_ this is not a bug that can be classified under unsafe
- orphan objects. like converting heap allocated objects to raw pointers and not deallocating them,
- proxy types (mutation of orphan object issue): drop is not properly implemented for a type which might contain an orphan object After an orphan object Box<&str> has been created, ptr is assigned to a proxy field. But, the default Drop implementation is ignorant that this field ought to be deallocated. \\
\textit{Hybrid analyser:}
- extracts the node order of graphs and eliminates loops
- encoder: information for heap values are encoded into bit vectors of fixed length . Analyses type definitions and further tries to use the already calculated vaues to mono-morphasise the code.
	- each type has a rtoken which can have values from abstract domain:
		- -1: unintialised,
		- 0: stack allocated/freed/moved
		- 1: heap allocated
	  \\
\textit{Model Checker:}
- input: hybrid analyser output
- model specifically designed to check leak free system using z3
\item\textbf{\ffichecker{}~\cite{inbook}:}  incorrect use of FFI:
	- heap memory is allocated in Rust and passed to C/C++.
	- two ways of passing a heap allocated value accross rust and C/C++.
		- (1) by borrowing the object as a reference- ownership with rust
		- (2) by moving the ownership to the FFI- rust forgets it and expects user to drop/free.
\textit{Static Analysis}
- Track status of all heap allocations: determine their borrow or moved status across cfgs
- heap allocations which cross FFI boundary are checked for being freed or not by external code

\textit{System Design:}
1. the user interface and driver program:
	1. convert user input to be suitable to tool like providing llvm bitcode and further. 
		1. downloads the dependent cargo/C files copies, sorts the source file for compilers and generates llvm bitcode
	2. works as a wrapper code for then, to facilitate interaction between various components
2. entry point and foreign function collector: determines entry point for static analysis. 
	1. collect the pub function and C/C++ called by rust: Implemented using HIR to get function name, visibility, implementation language(rust/C/C++)
3. the static analyser and bug detector: generates diagnostic messages after analysis
	1. Fixed point algorithm use of worklist algorithm to exhaustively analyse all basic blocks.
		1. Uses abstract interpretation for variables/blocks with heap allocation. for each basic block there a table is used to keep track of mappings
		2. Transfer functions: assigned to load/store/call, getelementptr llvm instructions
	2. For Call and invoke instruction: 
		- we categorize functions into different types:
            \begin{enumerate}
                \item Functions that allocate heap memory, e.g., exchange\_malloc.
		      \item Functions that borrow a reference (e.g., Vec::as\_mut\_ptr) or move the ownership (e.g., Box::into\_raw). change the abstract state of heap memory into either Borrowed/Move.
		      \item Foreign functions called through FFI. These are the potentially vulnerable functions that FFIChecker cares about. 
	        \item LLVM intrinsic functions and the Rust standard library functions - use of dummy functions to escape traversing them
            \end{enumerate}

\item\textbf{\safedrop{}} 
\textit{Types of bugs}
invalid memory deallocation by rust due to its ownership based model
	invalid drop in normal execution path and invalid drop  
in exception handling path.
	- use-after free
	- double free
\textit{Path Extraction}
- collects path by traversing a spanning tree. Spanning tree is formed using Tarjan's approach to merge the paths. 
- a valuable path should be a unique set of code blocks with a start node (function entrance) and an exit node
- the set of a valuable path should not be the subset of any other valuable  
paths.
#### Alias Analysis
- analyzes the alias relationship among the variables and the fields of the composite types for each data-flow.
- Does context insensitive interprocedural analysis by relating the alias with arg and return values
\textit{Invalid Drop detection}
- this step searches vulnerable drop patterns for each data-flow and records the suspicious code snippet
 \item\textbf{\rudra{}:}
\textit{Types of bugs}
- memory safety bugs in unsafe Rust
	- Panic Safety: drops the value of a type v in an unsafe or unexpected state like string should be utf-8 encoded but if a loop panics in between then the value will be dropped as non utf-8.
	- Higher-order Safety Invariant: caused by incorrectly assuming a higher-order invariant that is not guaranteed by the type system
	- Propagating Send/Sync in Generic Types
\textit{Bug Finding Algorithms}
\textit{ Unsafe dataflow checker} 
- uses taint tracking to track panic and higher order safety invariants
- checks for dataflows between lifetime bypasses and highly suspicious function calls (with panic() or high order parameter).
- At the MIR layer, uses an unresolvable generic function call as an approximation of a potential panic site or a location where higher-order invariants are implicitly assumed
\textit{Send/Sync variance checker:} still need to expand on this

\item\textbf{\lockbud{}:} 
% tool doesn't have a related paper need to analyse the source code

\end{itemize}
